Teaming up MET plus jet with Drell-Yan in the SMEFT

The Standard Model Effective Field Theory (SMEFT) is a widely utilized framework for exploring new physics effects in a model-independent manner. In previous studies, Drell-Yan collider data has emerged as a promising signature due to its energy enhancement relative to Standard Model predictions. We present recent works, extending this approach by also considering the "missing energy + jet" signature, which can constrain related dineutrino couplings and similarly benefits from energy enhancement. The combination of these observables allows for constraining a broader selection of operators and helps resolve flat directions in a global analysis. Overall, the bounds probe the multi-TeV range, with the strongest reaching up to $10\; \text{TeV}$ for four-fermion interactions and $7 \;\text{TeV}$ for gluonic dipole interactions. Furthermore, we find that low energy flavor observables improve limits by up to a factor of three for dipole operators. We also estimate sensitivities to new physics at future hadron colliders including the $\sqrt{s} = 27 \;\text{TeV}$ HE-LHC and the $\sqrt{s} = 100 \; \text{TeV}$ FCC-hh.

==> feynman/Goldstone.tex <==
\xdefinecolor{dRed}{RGB}{153, 0, 0}
\xdefinecolor{dOrange}{RGB}{251, 133, 0}
\xdefinecolor{dBlue}{RGB}{33, 158, 188}
\xdefinecolor{dGrey}{RGB}{100, 100, 100}

\begin{tikzpicture}[scale=1] \begin{feynman}
  
    \vertex [crossed dot](ww1){};
    % \vertex [right=2cm of c, small, blob, ] (ww1){};
    \vertex [left=1.cm of ww1] (ml);
    \vertex [right=1.cm of ww1] (mr);
    \vertex [above=0.7cm of ml] (u1);
    \vertex [left=0.3cm of u1] (u) {\(u^L_i\)};
    \vertex [below=0.7cm of ml] (u2);
    \vertex [left=0.3cm of u2] (u3) {\(g\)};
    \vertex [above=0.7cm of mr] (l1);
    \vertex [right=0.2cm of l1] (l) {\( u^R_j\)};
    \vertex [below=0.7cm of mr] (l2);
    \vertex [right=0.2cm of l2] (l3) {\(\pi^0\)};


    \vertex [right=4.0cm of ww1] (ww3){};
    \vertex [right=0.7cm of ww3] (ww4);
%
    \vertex[left=1cm of ww3] (ml2);
    \vertex[above=0.7cm of ml2] (gg1);
    \vertex[left=0.1cm of gg1] (g1) {\(u^L_i\)};
    \vertex[below=0.7cm of ml2] (qq1);
    \vertex[left=0.1cm of qq1] (q1) {\(g\)};
%%
    \vertex[right=1cm of ww4] (mr2);
    \vertex[above=0.7cm of mr2] (qq2);
    \vertex[right=0.1cm of qq2] (q2) {\(u^R_j\)};
%%
   \vertex[below=0.7cm of mr2] (h1);
   \vertex[right=0.2cm of mr2] (h2);
   \vertex[right=0.1cm of h1] (nubar) {$Z_L$};
   %\vertex[right=0.1cm of h2] (nu) {$\nu$};

   \vertex [right=4.0cm of ww4] (ww5);
   \vertex [right=0.7cm of ww5] (ww6);
%
   \vertex[left=1cm of ww5] (ml3){};
   \vertex[above=0.7cm of ml3] (gg2);
   \vertex[left=0.1cm of gg2] (g2) {\(u^L_i\)};
   \vertex[below=0.7cm of ml3] (qq2);
   \vertex[left=0.1cm of qq2] (q3) {\(g\)};
%%%

  \vertex[right=1.6cm of g2] (ww6);
  \vertex[right=1.5cm of q3] (ww7);
  \vertex[right= 1.5cm of ww6](g3){\(u^R_j\)};
  \vertex[right= 1.5cm of ww7](ZL){\(Z_L\)};
 %   \vertex[right=1cm of ww6] (mr3);
 %   \vertex[above=0.7cm of mr3] (qq3);
 %   \vertex[right=0.1cm of qq3] (q4) {\(q_j\)};
%%%
 %  \vertex[below=0.7cm of mr3] (h3);
 %  \vertex[right=0.2cm of mr3] (h4);
 %  \vertex[right=0.1cm of h3] (nubar2) {$Z_L$};

    \diagram* {
    (u) -- [thick,fermion] (ww1),
    (u3) -- [thick,gluon] (ww1),
    (l3) -- [thick,scalar] (ww1),
    (ww1) -- [thick,fermion ] (l),

   (ww3) -- [thick,fermion] (ww4) -- [thick, fermion] (q2),
   (gg1) -- [thick,fermion] (ww3),
   (qq1) -- [thick, gluon] (ww3),
    (ww4) -- [thick,boson] (h1),

    (g2) -- [thick,fermion] (ww6) -- [thick, boson] (ZL),
    (q3) -- [thick,gluon] (ww7),
    (ww7) -- [thick, fermion] (g3),
    (ww6) -- [thick,fermion] (ww7),

      };
  
      % \vertex [right=4.5cm of ww1] (ww2);
      %   % \vertex [right=2cm of c, small, blob, ] (ww1){};
      %   \vertex [left=1.cm of ww2] (ml2);
      %   \vertex [right=1.cm of ww2] (mr2);
      %   \vertex [above=0.7cm of ml2] (u12);
      %   \vertex [left=0.3cm of u12] (u4) {\(u\)};
      %   \vertex [below=0.7cm of ml2] (u22);
      %   \vertex [left=0.3cm of u22] (u32) {\(\bar c\)};

      %   \vertex [right=1.1cm of u4] (h1);
      %   \vertex [below=0.5cm of h1] (g1);
      %   \vertex [right=1.2cm of g1] (h2);
      %   \vertex [above=0.6cm of h2] (g2);

      %   \vertex [above=0.7cm of mr2] (l12);
      %   \vertex [right=0.2cm of l12] (l4) {\(\nu\)};
      %   \vertex [below=0.7cm of mr2] (l22);
      %   \vertex [right=0.2cm of l22] (l32) {\(\bar \nu \)};
  
    % \diagram* {
    % (u4) -- [thick,fermion] (ww2),
    % (ww2) -- [thick,fermion] (u32),
    % (l32) -- [thick,fermion] (ww2),
    % (ww2) -- [thick,fermion] (l4),
    % (g1) -- [thick,gluon] (g2),
    %   };
  
    \draw ( 2,0)node{$= $};
    \draw ( 6.7,0)node{$+$};
    \draw[fill = dBlue, dBlue ] (0,-0.0) circle (0.15) node[below = 5pt] {$C_{\underset{ij}{uG}}^{*} $};
    \draw[fill=dBlue, dBlue] (4,-0.0) circle (0.15) node[below = 5pt] {$C_{\underset{ij}{uG}}^{*} $};
    \draw[fill=dBlue, dBlue] (8.7,-0.7) circle (0.15) node[below right = 3pt] {$C_{\underset{ij}{uG}}^{*} $};

    \draw[fill = black, black ] (4.75,-0.0) circle (0.05) node[above = 5pt] {$\epsilon^u_R $};
    \draw[fill = black, black ] (8.7,0.7) circle (0.05) node[above = 5pt] {$\epsilon^u_L $};
  %
   % \draw (0.1,-0.7) node[ dOrange, font=\large] {};
   % \draw (4.8,-0.7) node[ dBlue, font=\large] {};

  
  
  \end{feynman} \end{tikzpicture}
  

==> feynman/Goldstone2.tex <==
\xdefinecolor{dRed}{RGB}{153, 0, 0}
\xdefinecolor{dOrange}{RGB}{251, 133, 0}
\xdefinecolor{dBlue}{RGB}{33, 158, 188}
\xdefinecolor{dGrey}{RGB}{100, 100, 100}

\begin{tikzpicture}[scale=1] \begin{feynman}
  
    \vertex [crossed dot](ww1){};
    % \vertex [right=2cm of c, small, blob, ] (ww1){};
    \vertex [left=1.cm of ww1] (ml);
    \vertex [right=1.cm of ww1] (mr);
    \vertex [above=0.7cm of ml] (u1);
    \vertex [left=0.3cm of u1] (u) {\(u^R_i\)};
    \vertex [below=0.7cm of ml] (u2);
    \vertex [left=0.3cm of u2] (u3) {\(g\)};
    \vertex [above=0.7cm of mr] (l1);
    \vertex [right=0.2cm of l1] (l) {\( u^L_j\)};
    \vertex [below=0.7cm of mr] (l2);
    \vertex [right=0.2cm of l2] (l3) {\(\pi^0\)};


    \vertex [right=4.0cm of ww1] (ww3){};
    \vertex [right=0.7cm of ww3] (ww4);
%
    \vertex[left=1cm of ww3] (ml2);
    \vertex[above=0.7cm of ml2] (gg1);
    \vertex[left=0.1cm of gg1] (g1) {\(u^R_i\)};
    \vertex[below=0.7cm of ml2] (qq1);
    \vertex[left=0.1cm of qq1] (q1) {\(g\)};
%%
    \vertex[right=1cm of ww4] (mr2);
    \vertex[above=0.7cm of mr2] (qq2);
    \vertex[right=0.1cm of qq2] (q2) {\(u^L_j\)};
%%
   \vertex[below=0.7cm of mr2] (h1);
   \vertex[right=0.2cm of mr2] (h2);
   \vertex[right=0.1cm of h1] (nubar) {$Z_L$};
   %\vertex[right=0.1cm of h2] (nu) {$\nu$};

   \vertex [right=4.0cm of ww4] (ww5);
   \vertex [right=0.7cm of ww5] (ww6);
%
   \vertex[left=1cm of ww5] (ml3){};
   \vertex[above=0.7cm of ml3] (gg2);
   \vertex[left=0.1cm of gg2] (g2) {\(u^R_i\)};
   \vertex[below=0.7cm of ml3] (qq2);
   \vertex[left=0.1cm of qq2] (q3) {\(g\)};
%%%

  \vertex[right=1.6cm of g2] (ww6);
  \vertex[right=1.5cm of q3] (ww7);
  \vertex[right= 1.5cm of ww6](g3){\(u^L_j\)};
  \vertex[right= 1.5cm of ww7](ZL){\(Z_L\)};
 %   \vertex[right=1cm of ww6] (mr3);
 %   \vertex[above=0.7cm of mr3] (qq3);
 %   \vertex[right=0.1cm of qq3] (q4) {\(q_j\)};
%%%
 %  \vertex[below=0.7cm of mr3] (h3);
 %  \vertex[right=0.2cm of mr3] (h4);
 %  \vertex[right=0.1cm of h3] (nubar2) {$Z_L$};

    \diagram* {
    (u) -- [thick,fermion] (ww1),
    (u3) -- [thick,gluon] (ww1),
    (l3) -- [thick,scalar] (ww1),
    (ww1) -- [thick,fermion ] (l),

   (ww3) -- [thick,fermion] (ww4) -- [thick, fermion] (q2),
   (gg1) -- [thick,fermion] (ww3),
   (qq1) -- [thick, gluon] (ww3),
    (ww4) -- [thick,boson] (h1),

    (g2) -- [thick,fermion] (ww6) -- [thick, boson] (ZL),
    (q3) -- [thick,gluon] (ww7),
    (ww7) -- [thick, fermion] (g3),
    (ww6) -- [thick,fermion] (ww7),

      };
  
      % \vertex [right=4.5cm of ww1] (ww2);
      %   % \vertex [right=2cm of c, small, blob, ] (ww1){};
      %   \vertex [left=1.cm of ww2] (ml2);
      %   \vertex [right=1.cm of ww2] (mr2);
      %   \vertex [above=0.7cm of ml2] (u12);
      %   \vertex [left=0.3cm of u12] (u4) {\(u\)};
      %   \vertex [below=0.7cm of ml2] (u22);
      %   \vertex [left=0.3cm of u22] (u32) {\(\bar c\)};

      %   \vertex [right=1.1cm of u4] (h1);
      %   \vertex [below=0.5cm of h1] (g1);
      %   \vertex [right=1.2cm of g1] (h2);
      %   \vertex [above=0.6cm of h2] (g2);

      %   \vertex [above=0.7cm of mr2] (l12);
      %   \vertex [right=0.2cm of l12] (l4) {\(\nu\)};
      %   \vertex [below=0.7cm of mr2] (l22);
      %   \vertex [right=0.2cm of l22] (l32) {\(\bar \nu \)};
  
    % \diagram* {
    % (u4) -- [thick,fermion] (ww2),
    % (ww2) -- [thick,fermion] (u32),
    % (l32) -- [thick,fermion] (ww2),
    % (ww2) -- [thick,fermion] (l4),
    % (g1) -- [thick,gluon] (g2),
    %   };
  
    \draw ( 2,0)node{$= $};
    \draw ( 6.7,0)node{$+$};
    \draw[fill = dBlue, dBlue ] (0,-0.0) circle (0.15) node[below = 5pt] {$C_{\underset{ji}{uG}} $};
    \draw[fill=dBlue, dBlue] (4,-0.0) circle (0.15) node[below = 5pt] {$C_{\underset{ji}{uG}} $};
    \draw[fill=dBlue, dBlue] (8.7,-0.7) circle (0.15) node[below right = 3pt] {$C_{\underset{ji}{uG}} $};

    \draw[fill = black, black ] (4.75,-0.0) circle (0.05) node[above = 5pt] {$\epsilon^u_L $};
    \draw[fill = black, black ] (8.7,0.7) circle (0.05) node[above = 5pt] {$\epsilon^u_R $};
  %
   % \draw (0.1,-0.7) node[ dOrange, font=\large] {};
   % \draw (4.8,-0.7) node[ dBlue, font=\large] {};

  
  
  \end{feynman} \end{tikzpicture}
  

==> feynman/dipoles.tex <==
\xdefinecolor{dRed}{RGB}{153, 0, 0}
\xdefinecolor{dOrange}{RGB}{251, 133, 0}
\xdefinecolor{dBlue}{RGB}{33, 158, 188}
\xdefinecolor{dGrey}{RGB}{100, 100, 100}

\begin{tikzpicture}[scale=1] \begin{feynman}


  \vertex (ww1);
    % \vertex [right=2cm of c, small, blob, ] (ww1){};
  \vertex [left=0.7cm of ww1] (ml);
  \vertex [right=1.cm of ww1] (gam);
  \vertex [right=0.7cm of gam] (mr);
  \vertex [above=0.7cm of ml] (u1);
  \vertex [left=0.3cm of u1] (u) {\(d\)};
  \vertex [below=0.7cm of ml] (u2);
  \vertex [left=0.3cm of u2] (u3) {\(\bar b\)};
  \vertex [above=0.7cm of mr] (l1);
  \vertex [right=0.2cm of l1] (l) {\(\ell^-\)};
  \vertex [below=0.7cm of mr] (l2);
  \vertex [right=0.2cm of l2] (l3) {\(\ell^+\)};


  \vertex [right=4.5cm of ww1] (ww3);
  \vertex [right=0.3cm of ww3] (ww13);
  \vertex [right=0.7cm of ww3] (ww4);

  \vertex[left=1cm of ww3] (ml2);
  \vertex[above=0.7cm of ml2] (gg1);
  \vertex[left=0.1cm of gg1] (g1) {g};
  \vertex[below=0.7cm of ml2] (qq1);
  \vertex[left=0.1cm of qq1] (q1) {\(d\)};

  \vertex[right=1cm of ww4] (mr2);
  \vertex[above=0.7cm of mr2] (qq2);
  \vertex[right=0.1cm of qq2] (q2) {\(b\)};
  \vertex[below=0.4cm of mr2] (h1);
  \vertex[left=0.3cm of h1] (Z);

  \vertex[right=0.7cm of Z] (mnu);
  \vertex[above=0.4cm of mnu] (nu1);
  \vertex[below=0.4cm of mnu] (nu2);
  \vertex[right=0.1cm of nu1] (nubar) {$\bar \nu$};
  \vertex[right=0.1cm of nu2] (nu) {$\nu$};


 

  \diagram* {
    (u) -- [thick,fermion] (ww1),
    (ww1) -- [thick,fermion] (u3),
    (ww1) -- [thick, boson, edge label=\({\gamma,Z}\)] (gam),
    (l3) -- [thick,fermion] (gam),
    (gam) -- [thick,fermion] (l),

    (ww3) -- [thick] (ww13) -- [thick,fermion] (ww4) -- [thick, fermion] (q2),
    (gg1) -- [thick,gluon] (ww3),
    (qq1) -- [thick, fermion] (ww3),
    (ww4) -- [thick, boson, edge label'=\({Z}\)] (Z),

    (nu1) -- [thick,fermion] (Z) -- [thick, fermion] (nu2),
      };


      \draw[fill=dOrange, dOrange] (0,-0.0) circle (0.15) node[right=5pt] {};
      \draw[fill=dBlue, dBlue] (5.2,0.0) circle (0.15) node[right=5pt] {}; 
    
      \draw (0.1,-0.8) node[ dOrange, font=\large] {$ C_{d \gamma/Z}$};
      \draw (5.0,0.5) node[ dBlue, font=\large] {$ C_{dZ}$};

  
  \end{feynman} \end{tikzpicture}
  



  
    % \vertex (ww1);
    % % \vertex [right=2cm of c, small, blob, ] (ww1){};
    % \vertex [left=0.7cm of ww1] (ml);
    % \vertex [right=1.cm of ww1] (gam);
    % \vertex [right=0.7cm of gam] (mr);
    % \vertex [above=0.7cm of ml] (u1);
    % \vertex [left=0.3cm of u1] (u) {\(u\)};
    % \vertex [below=0.7cm of ml] (u2);
    % \vertex [left=0.3cm of u2] (u3) {\(\bar c\)};
    % \vertex [above=0.7cm of mr] (l1);
    % \vertex [right=0.2cm of l1] (l) {\(l^-\)};
    % \vertex [below=0.7cm of mr] (l2);
    % \vertex [right=0.2cm of l2] (l3) {\(l^+\)};
  
    % \diagram* {
    % (u) -- [thick,fermion] (ww1),
    % (ww1) -- [thick,fermion] (u3),
    % (ww1) -- [thick, boson, edge label=\({\gamma,Z}\)] (gam),
    % (l3) -- [thick,fermion] (gam),
    % (gam) -- [thick,fermion] (l),
    %   };
  
    %   \vertex [right=4.9cm of ww1] (ww2);
    %     % \vertex [right=2cm of c, small, blob, ] (ww1){};
    %     \vertex [left=0.7cm of ww2] (ml2);
    %     \vertex [right=1.cm of ww2] (Z);
    %     \vertex [right=0.7cm of Z] (mr2);
    %     \vertex [above=0.7cm of ml2] (u12);
    %     \vertex [left=0.3cm of u12] (u4) {\(u\)};
    %     \vertex [below=0.7cm of ml2] (u22);
    %     \vertex [left=0.3cm of u22] (u32) {\(\bar c\)};

    %     \vertex [right=0.8cm of u4] (h1);
    %     \vertex [below=0.4cm of h1] (g1);
    %     \vertex [right=1.2cm of g1] (h2);
    %     \vertex [above=0.6cm of h2] (g2);

    %     \vertex [above=0.7cm of mr2] (l12);
    %     \vertex [right=0.2cm of l12] (l4) {\(\nu\)};
    %     \vertex [below=0.7cm of mr2] (l22);
    %     \vertex [right=0.2cm of l22] (l32) {\(\bar \nu \)};
  
    % \diagram* {
    % (u4) -- [thick,fermion] (ww2),
    % (ww2) -- [thick,fermion] (u32),
    % (l32) -- [thick,fermion] (Z),
    % (Z) -- [thick,fermion] (l4),
    % (g1) -- [thick,gluon] (g2),
    % (ww2) -- [thick, boson, edge label=\(Z\)] (Z),
    %   };
  
  
   
  

==> feynman/gluon_dipole.tex <==
\xdefinecolor{dRed}{RGB}{153, 0, 0}
\xdefinecolor{dOrange}{RGB}{251, 133, 0}
\xdefinecolor{dBlue}{RGB}{33, 158, 188}
\xdefinecolor{dGrey}{RGB}{100, 100, 100}

\begin{tikzpicture}[scale=1] \begin{feynman}

  \vertex (ww32);
  \vertex [right=0.3cm of ww32] (ww33);
  \vertex [right=0.7cm of ww32] (ww42);

  \vertex[left=1cm of ww32] (ml22);
  \vertex[above=0.7cm of ml22] (gg12);
  \vertex[left=0.1cm of gg12] (g12) {g};
  \vertex[below=0.7cm of ml22] (qq12);
  \vertex[left=0.1cm of qq12] (q12) {\(d\)};

  \vertex[right=1cm of ww42] (mr22);
  \vertex[above=0.7cm of mr22] (qq22);
  \vertex[right=0.1cm of qq22] (q22) {\(b\)};
  \vertex[below=0.4cm of mr22] (h12);
  \vertex[left=0.3cm of h12] (Z2);

  \vertex[right=0.7cm of Z2] (mnu2);
  \vertex[above=0.4cm of mnu2] (nu12);
  \vertex[below=0.4cm of mnu2] (nu22);
  \vertex[right=0.1cm of nu12] (nubar2) {$\bar \nu$};
  \vertex[right=0.1cm of nu22] (nu42) {$\nu$};


  \diagram* {

    (ww32) -- [thick] (ww33) -- [thick,fermion] (ww42) -- [thick, fermion] (q22),
    (gg12) -- [thick,gluon] (ww32),
    (qq12) -- [thick, fermion] (ww32),
    (ww42) -- [thick, boson, edge label'=\({Z}\)] (Z2),

    (nu12) -- [thick,fermion] (Z2) -- [thick, fermion] (nu22),
      };


      \draw (0.0,-0.7) node[ dBlue, font=\large] {$ C_{dG}$};

      \draw[fill=dBlue, dBlue] (0.0,-0.0) circle (0.15) node[right=5pt] {};

\end{feynman} \end{tikzpicture}

==> feynman/lq3.tex <==
\xdefinecolor{dRed}{RGB}{153, 0, 0}
\xdefinecolor{dOrange}{RGB}{251, 133, 0}
\xdefinecolor{dBlue}{RGB}{33, 158, 188}
\xdefinecolor{dGrey}{RGB}{100, 100, 100}

\begin{tikzpicture}[scale=1] \begin{feynman}
  
    \vertex (ww1);
    % \vertex [right=2cm of c, small, blob, ] (ww1){};
    \vertex [left=1.cm of ww1] (ml);
    \vertex [right=1.cm of ww1] (mr);
    \vertex [above=0.7cm of ml] (u1);
    \vertex [left=0.3cm of u1] (u) {\(d\)};
    \vertex [below=0.7cm of ml] (u2);
    \vertex [left=0.3cm of u2] (u3) {\(\bar b\)};
    \vertex [above=0.7cm of mr] (l1);
    \vertex [right=0.2cm of l1] (l) {\(\ell^-\)};
    \vertex [below=0.7cm of mr] (l2);
    \vertex [right=0.2cm of l2] (l3) {\(\ell^+\)};


    \vertex [right=4.0cm of ww1] (ww3);
    \vertex [right=0.7cm of ww3] (ww4);

    \vertex[left=1cm of ww3] (ml2);
    \vertex[above=0.7cm of ml2] (gg1);
    \vertex[left=0.1cm of gg1] (g1) {g};
    \vertex[below=0.7cm of ml2] (qq1);
    \vertex[left=0.1cm of qq1] (q1) {\(d\)};

    \vertex[right=1cm of ww4] (mr2);
    \vertex[above=0.7cm of mr2] (qq2);
    \vertex[right=0.1cm of qq2] (q2) {\(b\)};

    \vertex[below=0.7cm of mr2] (h1);
    \vertex[right=0.2cm of mr2] (h2);
    \vertex[right=0.1cm of h1] (nubar) {$\bar \nu$};
    \vertex[right=0.1cm of h2] (nu) {$\nu$};

  
    \diagram* {
    (u) -- [thick,fermion] (ww1),
    (ww1) -- [thick,fermion] (u3),
    (l3) -- [thick,fermion] (ww1),
    (ww1) -- [thick,fermion] (l),

    (ww3) -- [thick,fermion] (ww4) -- [thick, fermion] (q2),
    (gg1) -- [thick,gluon] (ww3),
    (qq1) -- [thick, fermion] (ww3),
    (h2) -- [thick,fermion] (ww4) -- [thick,fermion] (h1),
      };
  
      % \vertex [right=4.5cm of ww1] (ww2);
      %   % \vertex [right=2cm of c, small, blob, ] (ww1){};
      %   \vertex [left=1.cm of ww2] (ml2);
      %   \vertex [right=1.cm of ww2] (mr2);
      %   \vertex [above=0.7cm of ml2] (u12);
      %   \vertex [left=0.3cm of u12] (u4) {\(u\)};
      %   \vertex [below=0.7cm of ml2] (u22);
      %   \vertex [left=0.3cm of u22] (u32) {\(\bar c\)};

      %   \vertex [right=1.1cm of u4] (h1);
      %   \vertex [below=0.5cm of h1] (g1);
      %   \vertex [right=1.2cm of g1] (h2);
      %   \vertex [above=0.6cm of h2] (g2);

      %   \vertex [above=0.7cm of mr2] (l12);
      %   \vertex [right=0.2cm of l12] (l4) {\(\nu\)};
      %   \vertex [below=0.7cm of mr2] (l22);
      %   \vertex [right=0.2cm of l22] (l32) {\(\bar \nu \)};
  
    % \diagram* {
    % (u4) -- [thick,fermion] (ww2),
    % (ww2) -- [thick,fermion] (u32),
    % (l32) -- [thick,fermion] (ww2),
    % (ww2) -- [thick,fermion] (l4),
    % (g1) -- [thick,gluon] (g2),
    %   };
  
  
    \draw[fill=dOrange, dOrange] (0,-0.0) circle (0.15) node[right=5pt] {};
    \draw[fill=dBlue, dBlue] (4.85,-0.0) circle (0.15) node[right=5pt] {};
  
    \draw (0.1,-0.7) node[ dOrange, font=\large] {$ C_{lq}^{+}$};
    \draw (4.8,-0.7) node[ dBlue, font=\large] {$ C_{lq}^{-}$};
  
  
  
  \end{feynman} \end{tikzpicture}
  
